Strange-metal behavior without fine-tuning in PrV2Al20

Strange-metal behavior observed in the praseodymium-based heavy-fermion material PrV2Al20 has been tentatively interpreted in the framework of proximity to a quantum critical point (QCP) associated with quadrupolar ordering. Here, we demonstrate that an alternative, natural explanation exists without invoking a QCP, in terms of the unconventional nature of the quadrupolar Kondo effect taking place in non-Kramers ions. Using a combination of ab initio density-functional theory calculations and analytical arguments, we construct a periodic Anderson model with realistic parameters to describe PrV2Al20. We solve the model using dynamical mean-field theory preserving the model symmetries and demonstrate the non-Fermi liquid strange-metal behavior stemming from the two-channel nature of the quadrupolar Kondo effect. Our calculations provide an explanation for the puzzling temperature dependence in the magnetic susceptibility, and provide a basis for analyzing future photoemission experiments.

==> preamble.tex <==
\newlength{\stumplen}
\setlength{\stumplen}{2cm}
\newlength{\bubblesize}
\setlength{\bubblesize}{2.5cm}

\newcommand{\intinf}[1]{{\ensuremath \int_{-\infty}^{\infty} d #1 \;}}
\newcommand{\Xint}[1]{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\newcommand{\XXint}[3]{{\setbox0=\hbox{$#1{#2#3}{\int}$}
     \vcenter{\hbox{$#2#3$}}\kern-.6\wd0}}
\newcommand{\pint}{\Xint{\mathcal{P}}}
\newcommand{\pintinf}[1]{{\ensuremath \; \pint_{-\infty}^{\infty} d #1 \;}}
% \newcommand{\real}{{\ensuremath \mathcal{R} \,}}
% \newcommand{\imag}{{\ensuremath \mathcal{I} \,}}
\newcommand{\real}{{\ensuremath \operatorname{Re} \,}}
\newcommand{\imag}{{\ensuremath \operatorname{Im} \,}}
\newcommand{\sgn}{{\ensuremath \operatorname{sgn}}}
\newcommand{\fullg}{{\ensuremath \mathcal{G}}}
\newcommand{\mtx}[4]{{\ensuremath \begin{pmatrix}#1 & #2\\ #3 & #4\end{pmatrix}}}
\newcommand{\dphant}{{\ensuremath{\vphantom{\dagger}}}}
\newcommand*{\Tr}[1]{\ensuremath{\text{Tr}\left( #1 \right)}}
\newcommand*{\tr}[1]{\ensuremath{\text{tr}\left( #1 \right)}}
\newcommand{\expect}[1]{{\ensuremath{\langle #1 \rangle}}}
\newcommand{\mylblue}{green!40!blue!70}
\newcommand{\myred}{red!50!white!70}
\newcommand{\vkt}{\ensuremath{\Tilde{\vk}}}
\newcommand{\vx}{\ensuremath{\vec{x}}}
\newcommand{\pprime}{\ensuremath{{\prime \prime}}}
\newcommand{\ppprime}{\ensuremath{{\prime \prime \prime}}}
\newcommand{\pppprime}{\ensuremath{{\prime \prime \prime \prime}}}
\newcommand{\bG}{\ensuremath{\boldsymbol{G}}}
\newcommand{\bV}{\ensuremath{\boldsymbol{V}}}
\newcommand{\bfG}{\ensuremath{\boldsymbol{\fullg}}}
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\atanh}{atanh}
\DeclareMathOperator{\atan}{atan}
\newcommand*{\barbI}[1]{\stackunder[1.0pt]{$#1$}{\rule{0.9ex}{0.095ex}}} 
\newcommand*{\barbII}[1]{\barbI{\barbI{#1}}}
